Multi-timescale reverberation mapping of Mrk 335

Time lags due to X-ray reverberation have been detected in several Seyfert galaxies. The different travel time between reflected and directly observed rays naturally causes this type of lag, which depends directly on the light-crossing timescale of the system and hence scales with the mass of the central black hole. Featureless `hard lags' not associated with reverberation, and often interpreted as propagating mass accretion rate fluctuations, dominate the longer timescale variability. Here we fit our reltrans model simultaneously to the time-averaged energy spectrum and the lag-energy spectra of the Seyfert galaxy Mrk 335 over two timescales (Fourier frequency ranges). We model the hard lags as fluctuations in the slope and strength of the illuminating spectrum, and self-consistently account for the effects that these fluctuations have on the reverberation lags. The resulting mass estimate is $1.1^{+2.0}_{-0.7} \times 10^6~M_\odot$, which is significantly lower than the mass measured with the optical reverberation mapping technique (14 - 26 million $M_\odot$). When we add the correlated variability amplitudes to the time lags by fitting the full complex cross-spectra, the model is unable to describe the characteristic reverberation Fe K$\alpha$ line and cannot constrain the black hole mass. This may be due to the assumption that the direct radiation is emitted by a point-like source.

==> library_2020.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created by Guglielmo Mastroserio 

%% Saved with string encoding Unicode (UTF-8) 

\AtBeginDocument{\renewcommand{\harvardand}{e}}

@string{aanda = {A\&A}}

@string{aandal = {A\&A}}

@string{aj = {AJ}}

@string{apj = {ApJ}}

@string{apjl = {ApJ}}

@string{apjs = {ApJ}}

@string{araa = {ARA\&A}}

@string{mnras = {MNRAS}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{Haardt1991,
       author = {{Haardt}, F. and {Maraschi}, L.},
        title = "{A Two-Phase Model for the X-Ray Emission from Seyfert Galaxies}",
      journal = {\apjl},
     keywords = {Accretion Disks, Astronomical Models, Emission Spectra, Seyfert Galaxies, X Ray Spectra, Computational Astrophysics, Galactic Nuclei, Gravitational Effects, Interstellar Magnetic Fields, Magnetic Field Reconnection, Astrophysics, GALAXIES: NUCLEI, X-RAYS: SPECTRA},
         year = "1991",
        month = "Oct",
       volume = {380},
        pages = {L51},
          doi = {10.1086/186171},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991ApJ...380L..51H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Haardt1993,
       author = {{Haardt}, Francesco and {Maraschi}, Laura},
        title = "{X-Ray Spectra from Two-Phase Accretion Disks}",
      journal = {\apj},
     keywords = {Accretion Disks, Active Galactic Nuclei, Compton Effect, Electron Energy, Stellar Luminosity, X Ray Spectra, Astronomical Models, Black Body Radiation, Stellar Coronas, X Ray Astronomy, Astrophysics, GALAXIES: ACTIVE, X-RAYS: GALAXIES, ACCRETION, ACCRETION DISKS},
         year = "1993",
        month = "Aug",
       volume = {413},
        pages = {507},
          doi = {10.1086/173020},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ApJ...413..507H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reynolds2014,
       author = {{Reynolds}, Christopher S.},
        title = "{Measuring Black Hole Spin Using X-Ray Reflection Spectroscopy}",
      journal = {\ssr},
     keywords = {Accretion disks, Black holes, X-ray astronomy, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
         year = "2014",
        month = "Sep",
       volume = {183},
       number = {1-4},
        pages = {277-294},
          doi = {10.1007/s11214-013-0006-6},
archivePrefix = {arXiv},
       eprint = {1302.3260},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014SSRv..183..277R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lightman1988,
       author = {{Lightman}, Alan P. and {White}, Timothy R.},
        title = "{Effects of Cold Matter in Active Galactic Nuclei: A Broad Hump in the X-Ray Spectra}",
      journal = {\apj},
     keywords = {Active Galactic Nuclei, Astronomical Spectroscopy, Dark Matter, Spectral Energy Distribution, X Ray Spectra, Black Holes (Astronomy), Optical Thickness, Spectrum Analysis, Astrophysics, GALAXIES: NUCLEI, X-RAYS: SPECTRA},
         year = "1988",
        month = "Dec",
       volume = {335},
        pages = {57},
          doi = {10.1086/166905},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988ApJ...335...57L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Fabian2000,
       author = {{Fabian}, A.~C. and {Iwasawa}, K. and {Reynolds}, C.~S. and
         {Young}, A.~J.},
        title = "{Broad Iron Lines in Active Galactic Nuclei}",
      journal = {\pasp},
     keywords = {accretion, accretion disks, black hole physics, Galaxies: Active, line: formation, line: profiles, X-rays: galaxies, Astrophysics},
         year = "2000",
        month = "Sep",
       volume = {112},
       number = {775},
        pages = {1145-1161},
          doi = {10.1086/316610},
archivePrefix = {arXiv},
       eprint = {astro-ph/0004366},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000PASP..112.1145F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Shields1978,
       author = {{Shields}, G.~A.},
        title = "{Thermal continuum from accretion disks in quasars}",
      journal = {\nat},
     keywords = {Continuous Spectra, Quasars, Stellar Mass Accretion, Thermal Emission, Seyfert Galaxies, Astrophysics},
         year = "1978",
        month = "Apr",
       volume = {272},
       number = {5655},
        pages = {706-708},
          doi = {10.1038/272706a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1978Natur.272..706S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Malkan1983,
       author = {{Malkan}, M.~A.},
        title = "{The ultraviolet excess of luminous quasars. II. Evidence for massive accretion disks.}",
      journal = {\apj},
     keywords = {Accretion Disks, Astronomical Models, Quasars, Seyfert Galaxies, Ultraviolet Spectra, Angular Momentum, Black Holes (Astronomy), Infrared Spectra, Luminosity, Relativity, Spectrum Analysis, Astrophysics},
         year = "1983",
        month = "May",
       volume = {268},
        pages = {582-590},
          doi = {10.1086/160981},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983ApJ...268..582M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%********************************************* PROCEEDINGS *********************************************

@INPROCEEDINGS{Novikov1973,
       author = {{Novikov}, I.~D. and {Thorne}, K.~S.},
        title = "{Astrophysics of black holes.}",
    booktitle = {Black Holes (Les Astres Occlus)},
         year = 1973,
        month = jan,
        pages = {343-450},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1973blho.conf..343N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Klis1989,
	author = {{van der Klis}, M.},
	title = "{Fourier techniques in X-ray timing}",
	keywords = {X-Ray Pulsars: Periods, X-Ray Pulsars: Power Spectra},
	booktitle = {NATO Advanced Science Institutes (ASI) Series C},
	year = 1989,
	series = {NATO Advanced Science Institutes (ASI) Series C},
	volume = 262,
	editor = {{{\"O}gelman}, H. and {van den Heuvel}, E.~P.~J.},
	pages = {27},
	adsurl = {http://adsabs.harvard.edu/abs/1989ASIC..262...27V},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Arnaud1996,
	author = {{Arnaud}, K.~A.},
	title = "{XSPEC: The First Ten Years}",
	booktitle = {Astronomical Data Analysis Software and Systems V},
	year = 1996,
	series = {Astronomical Society of the Pacific Conference Series},
	volume = 101,
	editor = {{Jacoby}, G.~H. and {Barnes}, J.},
	pages = {17},
	adsurl = {http://adsabs.harvard.edu/abs/1996ASPC..101...17A},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Garcia2018,
       author = {{Garc{\'\i}a}, J.~A. and {Kallman}, T.~R. and {Bautista}, M. and
         {Mendoza}, C. and {Deprince}, J. and {Palmeri}, P. and {Quinet}, P.},
        title = "{The Problem of the High Iron Abundance in Accretion Disks around Black Holes}",
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
    booktitle = {Workshop on Astrophysical Opacities},
         year = "2018",
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {515},
        month = "Aug",
        pages = {282},
archivePrefix = {arXiv},
       eprint = {1805.00581},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ASPC..515..282G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Huppenkothen2016,
       author = {{Huppenkothen}, Daniela},
        title = "{(Bayesian) Inference for X-ray Timing}",
    booktitle = {41st COSPAR Scientific Assembly},
         year = "2016",
       volume = {41},
        month = "Jul",
          eid = {E1.1-109-16},
        pages = {E1.1-109-16},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016cosp...41E.850H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%********************************************* BOOKS *********************************************
@ARTICLE{Bendat2000,
       author = {{Bendat}, J.~S. and {Piersol}, A.~G.},
        title = "{BOOK REVIEW:  Random Data Analysis and Measurement Procedures}",
      journal = {Measurement Science and Technology},
         year = "2000",
        month = "Dec",
       volume = {11},
       number = {12},
        pages = {1825-1826},
          doi = {10.1088/0957-0233/11/12/702},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000MeScT..11.1825B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{Oppenheim1975,
	author = {{Oppenheim}, A.~V. and {Schafer}, R.~W.},
	title = "{Digital signal processing}",
	booktitle = {Digital Signal Processing},
	year = 1975,
	adsurl = {http://adsabs.harvard.edu/abs/1975dsp..book.....O},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%********************************************* ARTICLES *********************************************

@ARTICLE{Arevalo2006,
	author = {{Ar{\'e}valo}, P. and {Uttley}, P.},
	title = "{Investigating a fluctuating-accretion model for the spectral-timing properties of accreting black hole systems}",
	journal = {\mnras},
	eprint = {astro-ph/0512394},
	keywords = {accretion, accretion discs, galaxies: active},
	year = 2006,
	month = apr,
	volume = 367,
	pages = {801-814},
	doi = {10.1111/j.1365-2966.2006.09989.x},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.367..801A},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Axelsson2013,
	author = {{Axelsson}, M. and {Hjalmarsdotter}, L. and {Done}, C.},
	title = "{Fast variability as a probe of the smallest regions around accreting black holes}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1301.0627},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual: XTE J1550-564},
	year = 2013,
	month = may,
	volume = 431,
	pages = {1987-1994},
	doi = {10.1093/mnras/stt315},
	adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.431.1987A},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Basak2017,
	author = {{Basak}, R. and {Zdziarski}, A.~A. and {Parker}, M. and {Islam}, N.
	},
	title = "{Analysis of NuSTAR and Suzaku observations of Cyg X-1 in the hard state: evidence for a truncated disc geometry}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1705.06638},
	primaryClass = "astro-ph.HE",
	keywords = {Astrophysics - High Energy Astrophysical Phenomena},
	year = 2017,
	month = may,
	adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170506638B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cackett2014,
	author = {{Cackett}, E.~M. and {Zoghbi}, A. and {Reynolds}, C. and {Fabian}, A.~C. and 
	{Kara}, E. and {Uttley}, P. and {Wilkins}, D.~R.},
	title = "{Modelling the broad Fe K{$\alpha$} reverberation in the AGN NGC 4151}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1311.2997},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, galaxies: active, galaxies: Seyfert, X-rays: galaxies, X-rays: individual: NGC 4151},
	year = 2014,
	month = mar,
	volume = 438,
	pages = {2980-2994},
	doi = {10.1093/mnras/stt2424},
	adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438.2980C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Campana1995,
	author = {{Campana}, S. and {Stella}, L.},
	title = "{Reverberation by a relativistic accretion disc}",
	journal = {\mnras},
	eprint = {astro-ph/9409049},
	keywords = {ACCRETION, ACCRETION DISCS-LINE, FORMATION-GALAXIES, NUCLEI-GALAXIES, SEYFERT-X-RAYS, GALAXIES.},
	year = 1995,
	month = feb,
	volume = 272,
	pages = {585-598},
	doi = {10.1093/mnras/272.3.585},
	adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.272..585C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Casares2014,
   author = {{Casares}, J. and {Jonker}, P.~G.},
    title = "{Mass Measurements of Stellar and Intermediate-Mass Black Holes}",
  journal = {\ssr},
archivePrefix = "arXiv",
   eprint = {1311.5118},
 primaryClass = "astro-ph.HE",
 keywords = {Black holes, X-ray binaries, Accretion disks},
     year = 2014,
    month = sep,
   volume = 183,
    pages = {223-252},
      doi = {10.1007/s11214-013-0030-6},
   adsurl = {http://adsabs.harvard.edu/abs/2014SSRv..183..223C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chainakun2016a,
	author = {{Chainakun}, P. and {Young}, A.~J. and {Kara}, E.},
	title = "{Relativistic X-ray reverberation modelling of the combined time-averaged and lag-energy spectra in AGN}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1605.01300},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, galaxies: active, galaxies: individual: Ark 564, galaxies: individual: IRAS 13224-3809, galaxies: individual: Mrk 335, X-rays: galaxies},
	year = 2016,
	month = aug,
	volume = 460,
	pages = {3076-3088},
	doi = {10.1093/mnras/stw1105},
	adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.460.3076C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chainakun2017,
	author = {{Chainakun}, P. and {Young}, A.~J.},
	title = "{Investigating the X-ray time lags in PG 1244+026 using an extended corona model}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1611.04396},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, black hole physics, galaxies: active, galaxies: individual: PG 1244+026, X-rays: galaxies},
	year = 2017,
	month = mar,
	volume = 465,
	pages = {3965-3976},
	doi = {10.1093/mnras/stw2964},
	adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.465.3965C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chainakun2019,
       author = {{Chainakun}, P. and {Watcharangkool}, A. and {Young}, A.~J. and
         {Hancock}, S.},
        title = "{X-ray time lags in AGN: inverse-Compton scattering and spherical corona model}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, galaxies: active, galaxies: individual: 1H0707-495, galaxies: individual: Ark 564, galaxies: individual: NGC 4051, galaxies: individual: IRAS 13224-3809, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Jul",
       volume = {487},
       number = {1},
        pages = {667-680},
          doi = {10.1093/mnras/stz1319},
archivePrefix = {arXiv},
       eprint = {1905.03683},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.487..667C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Coppi1999,
	author = {{Coppi}, P.~S.},
	title = "{The Physics of Hybrid Thermal/Non-Thermal Plasmas}",
	booktitle = {High Energy Processes in Accreting Black Holes},
	year = 1999,
	series = {Astronomical Society of the Pacific Conference Series},
	volume = 161,
	eprint = {astro-ph/9903158},
	editor = {{Poutanen}, J. and {Svensson}, R.},
	pages = {375},
	adsurl = {http://adsabs.harvard.edu/abs/1999ASPC..161..375C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dauser2012,
       author = {{Dauser}, T. and {Svoboda}, J. and {Schartel}, N. and {Wilms}, J. and
         {Dov{\v{c}}iak}, M. and {Ehle}, M. and {Karas}, V. and
         {Santos-Lle{\'o}}, M. and {Marshall}, H.~L.},
        title = "{Spectral analysis of 1H 0707-495 with XMM-Newton}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: individual: 1H 0707-495, galaxies: nuclei, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "May",
       volume = {422},
       number = {3},
        pages = {1914-1921},
          doi = {10.1111/j.1365-2966.2011.20356.x},
archivePrefix = {arXiv},
       eprint = {1112.1796},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.422.1914D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dauser2013,
   author = {{Dauser}, T. and {Garcia}, J. and {Wilms}, J. and {B{\"o}ck}, M. and 
	{Brenneman}, L.~W. and {Falanga}, M. and {Fukumura}, K. and 
	{Reynolds}, C.~S.},
    title = "{Irradiation of an accretion disc by a jet: general properties and implications for spin measurements of black holes}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1301.4922},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, black hole physics, lines: profiles, galaxies: active, galaxies: nuclei},
     year = 2013,
    month = apr,
   volume = 430,
    pages = {1694-1708},
      doi = {10.1093/mnras/sts710},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.430.1694D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeMarco2013b,
   author = {{De Marco}, B. and {Ponti}, G. and {Cappi}, M. and {Dadina}, M. and 
	{Uttley}, P. and {Cackett}, E.~M. and {Fabian}, A.~C. and {Miniutti}, G.
	},
    title = "{Discovery of a relation between black hole mass and soft X-ray time lags in active galactic nuclei}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1201.0196},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: active, galaxies: nuclei, X-rays: galaxies},
     year = 2013,
    month = may,
   volume = 431,
    pages = {2441-2452},
      doi = {10.1093/mnras/stt339},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.431.2441D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeMarco2013a,
   author = {{De Marco}, B. and {Ponti}, G. and {Miniutti}, G. and {Belloni}, T. and 
	{Cappi}, M. and {Dadina}, M. and {Mu{\~n}oz-Darias}, T.},
    title = "{Time lags in the ultraluminous X-ray source NGC 5408 X-1: implications for the black hole mass}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1310.0042},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, black hole physics, X-rays: individual: NGC 5408 X-1},
     year = 2013,
    month = dec,
   volume = 436,
    pages = {3782-3791},
      doi = {10.1093/mnras/stt1853},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.436.3782D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeMarco2015,
	author = {{De Marco}, B. and {Ponti}, G. and {Mu{\~n}oz-Darias}, T. and 
	{Nandra}, K.},
	title = "{Tracing the Reverberation Lag in the Hard State of Black Hole X-Ray Binaries}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1510.02798},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion disks, black hole physics, X-rays: binaries},
	year = 2015,
	month = nov,
	volume = 814,
	eid = {50},
	pages = {50},
	doi = {10.1088/0004-637X/814/1/50},
	adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...814...50D},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeMarco2016,
	author = {{De Marco}, B. and {Ponti}, G.},
	title = "{The Reverberation Lag in the Low-mass X-ray Binary H1743-322}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1605.00765},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion disks, X-rays: binaries, X-rays: individual: H1743-322},
	year = 2016,
	month = jul,
	volume = 826,
	eid = {70},
	pages = {70},
	doi = {10.3847/0004-637X/826/1/70},
	adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...826...70D},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{DeMarco2017,
	author = {{De Marco}, B. and {Ponti}, G. and {Petrucci}, P.~O. and {Clavel}, M. and 
	{Corbel}, S. and {Belmont}, R. and {Chakravorty}, S. and {Coriat}, M. and 
	{Drappeau}, S. and {Ferreira}, J. and {Henri}, G. and {Malzac}, J. and 
	{Rodriguez}, J. and {Tomsick}, J.~A. and {Ursini}, F. and {Zdziarski}, A.~A.
	},
	title = "{Evolution of the reverberation lag in GX 339-4 at the end of an outburst}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1706.10053},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual: GX 3394},
	year = 2017,
	month = oct,
	volume = 471,
	pages = {1475-1487},
	doi = {10.1093/mnras/stx1649},
	adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.471.1475D},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Done2007,
       author = {{Done}, Chris and {Gierli{\'n}ski}, Marek and {Kubota}, Aya},
        title = "{Modelling the behaviour of accretion flows in X-ray binaries. Everything you always wanted to know about accretion but were afraid to ask}",
      journal = {\aapr},
     keywords = {Accretion, accretion discs, Black hole physics, X-rays: binaries, Astrophysics},
         year = "2007",
        month = "Dec",
       volume = {15},
       number = {1},
        pages = {1-66},
          doi = {10.1007/s00159-007-0006-1},
archivePrefix = {arXiv},
       eprint = {0708.0148},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&ARv..15....1D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Done2012,
	author = {{Done}, C. and {Davis}, S.~W. and {Jin}, C. and {Blaes}, O. and 
	{Ward}, M.},
	title = "{Intrinsic disc emission and the soft X-ray excess in active galactic nuclei}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1107.5429},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, black hole physics, galaxies: active},
	year = 2012,
	month = mar,
	volume = 420,
	pages = {1848-1860},
	doi = {10.1111/j.1365-2966.2011.19779.x},
	adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.420.1848D},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Duro2016,
	author = {{Duro}, R. and {Dauser}, T. and {Grinberg}, V. and {Mi{\v s}kovi{\v c}ov{\'a}}, I. and 
	{Rodriguez}, J. and {Tomsick}, J. and {Hanke}, M. and {Pottschmidt}, K. and 
	{Nowak}, M.~A. and {Kreykenbohm}, S. and {Cadolle Bel}, M. and 
	{Bodaghee}, A. and {Lohfink}, A. and {Reynolds}, C.~S. and {Kendziorra}, E. and 
	{Kirsch}, M.~G.~F. and {Staubert}, R. and {Wilms}, J.},
	title = "{Revealing the broad iron K{$\alpha$} line in Cygnus X-1 through simultaneous XMM-Newton, RXTE, and INTEGRAL observations}",
	journal = {\aap},
	archivePrefix = "arXiv",
	eprint = {1602.08756},
	primaryClass = "astro-ph.HE",
	keywords = {X-rays: binaries, black hole physics, gravitation},
	year = 2016,
	month = may,
	volume = 589,
	eid = {A14},
	pages = {A14},
	doi = {10.1051/0004-6361/201424740},
	adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...589A..14D},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eardley1975,
	author = {{Eardley}, D.~M. and {Lightman}, A.~P. and {Shapiro}, S.~L.},
	title = "{Cygnus X-1 - A two-temperature accretion disk model which explains the observed hard X-ray spectrum}",
	journal = {\apjl},
	keywords = {Astronomical Models, Binary Stars, Black Holes (Astronomy), Stellar Temperature, X Ray Spectra, X Ray Stars, Radiant Flux Density, Stellar Evolution, Stellar Spectra, X Ray Astronomy},
	year = 1975,
	month = aug,
	volume = 199,
	pages = {L153-L155},
	doi = {10.1086/181871},
	adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...199L.153E},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Edelson2019,
       author = {{Edelson}, R. and {Gelbord}, J. and {Cackett}, E. and {Peterson}, B.~M. and
         {Horne}, K. and {Barth}, A.~J. and {Starkey}, D.~A. and {Bentz}, M. and
         {Brandt}, W.~N. and {Goad}, M. and {Joner}, M. and {Korista}, K. and
         {Netzer}, H. and {Page}, K. and {Uttley}, P. and {Vaughan}, S. and
         {Breeveld}, A. and {Cenko}, S.~B. and {Done}, C. and {Evans}, P. and
         {Fausnaugh}, M. and {Ferland}, G. and {Gonzalez-Buitrago}, D. and
         {Gropp}, J. and {Grupe}, D. and {Kaastra}, J. and {Kennea}, J. and
         {Kriss}, G. and {Mathur}, S. and {Mehdipour}, M. and {Mudd}, D. and
         {Nousek}, J. and {Schmidt}, T. and {Vestergaard}, M. and
         {Villforth}, C.},
        title = "{The First Swift Intensive AGN Accretion Disk Reverberation Mapping Survey}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = jan,
       volume = {870},
       number = {2},
          eid = {123},
        pages = {123},
          doi = {10.3847/1538-4357/aaf3b4},
archivePrefix = {arXiv},
       eprint = {1811.07956},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...870..123E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eijnden2017,
	author = {{van den Eijnden}, J. and {Ingram}, A. and {Uttley}, P. and 
	{Motta}, S.~E. and {Belloni}, T.~M. and {Gardenier}, D.~W.},
	title = "{Inclination dependence of QPO phase lags in black hole X-ray binaries}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1610.03469},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, black hole physics, X-rays: binaries},
	year = 2017,
	month = jan,
	volume = 464,
	pages = {2643-2659},
	doi = {10.1093/mnras/stw2634},
	adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.464.2643V},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Emmanoulopoulos2014,
	author = {{Emmanoulopoulos}, D. and {Papadakis}, I.~E. and {Dov{\v c}iak}, M. and 
	{McHardy}, I.~M.},
	title = "{General relativistic modelling of the negative reverberation X-ray time delays in AGN}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1402.0899},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, black hole physics, relativistic processes, galaxies: active, galaxies: nuclei, X-rays: galaxies},
	year = 2014,
	month = apr,
	volume = 439,
	pages = {3931-3950},
	doi = {10.1093/mnras/stu249},
	adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.439.3931E},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Epitropakis2016a,
       author = {{Epitropakis}, A. and {Papadakis}, I.~E.},
        title = "{Statistical properties of Fourier-based time-lag estimates}",
      journal = {\aap},
     keywords = {methods: statistical, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = jun,
       volume = {591},
          eid = {A113},
        pages = {A113},
          doi = {10.1051/0004-6361/201527665},
archivePrefix = {arXiv},
       eprint = {1604.01726},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...591A.113E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Epitropakis2016,
	author = {{Epitropakis}, A. and {Papadakis}, I.~E. and {Dov{\v c}iak}, M. and 
	{Pech{\'a}{\v c}ek}, T. and {Emmanoulopoulos}, D. and {Karas}, V. and 
	{McHardy}, I.~M.},
	title = "{Theoretical modelling of the AGN iron line vs. continuum time-lags in the lamp-post geometry}",
	journal = {\aap},
	archivePrefix = "arXiv",
	eprint = {1607.02625},
	primaryClass = "astro-ph.HE",
	keywords = {galaxies: active, X-rays: galaxies, accretion, accretion disks, galaxies: Seyfert, relativistic processes},
	year = 2016,
	month = oct,
	volume = 594,
	eid = {A71},
	pages = {A71},
	doi = {10.1051/0004-6361/201527748},
	adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...594A..71E},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Epitropakis2017,
	author = {{Epitropakis}, A. and {Papadakis}, I.~E.},
	title = "{The X-ray continuum time-lags and intrinsic coherence in AGN}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1703.04322},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, relativistic processes, galaxies: active, galaxies: Seyfert, X-rays: galaxies},
	year = 2017,
	month = jul,
	volume = 468,
	pages = {3568-3601},
	doi = {10.1093/mnras/stx612},
	adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.468.3568E},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Esin1997,
       author = {{Esin}, Ann A. and {McClintock}, Jeffrey E. and {Narayan}, Ramesh},
        title = "{Advection-Dominated Accretion and the Spectral States of Black Hole X-Ray Binaries: Application to Nova Muscae 1991}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, X-rays: stars, Astrophysics},
         year = "1997",
        month = "Nov",
       volume = {489},
       number = {2},
        pages = {865-889},
          doi = {10.1086/304829},
archivePrefix = {arXiv},
       eprint = {astro-ph/9705237},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...489..865E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fabian1989,
	author = {{Fabian}, A.~C. and {Rees}, M.~J. and {Stella}, L. and {White}, N.~E.
	},
	title = "{X-ray fluorescence from the inner disc in Cygnus X-1}",
	journal = {\mnras},
	keywords = {Accretion Disks, Black Holes (Astronomy), Cygnus Constellation, X Ray Fluorescence, X Ray Spectra, Black Body Radiation, Emission Spectra, Line Spectra, Red Shift},
	year = 1989,
	month = may,
	volume = 238,
	pages = {729-736},
	doi = {10.1093/mnras/238.3.729},
	adsurl = {http://adsabs.harvard.edu/abs/1989MNRAS.238..729F},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fabian2009,
   author = {{Fabian}, A.~C. and {Zoghbi}, A. and {Ross}, R.~R. and {Uttley}, P. and 
	{Gallo}, L.~C. and {Brandt}, W.~N. and {Blustin}, A.~J. and 
	{Boller}, T. and {Caballero-Garcia}, M.~D. and {Larsson}, J. and 
	{Miller}, J.~M. and {Miniutti}, G. and {Ponti}, G. and {Reis}, R.~C. and 
	{Reynolds}, C.~S. and {Tanaka}, Y. and {Young}, A.~J.},
    title = "{Broad line emission from iron K- and L-shell transitions in the active galaxy 1H0707-495}",
  journal = {\nat},
     year = 2009,
    month = may,
   volume = 459,
    pages = {540-542},
      doi = {10.1038/nature08007},
   adsurl = {http://adsabs.harvard.edu/abs/2009Natur.459..540F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fabian2010,
   author = {{Fabian}, A.~C. and {Ross}, R.~R.},
    title = "{X-ray Reflection}",
  journal = {\ssr},
 keywords = {X-ray astronomy, Radiation processes},
     year = 2010,
    month = dec,
   volume = 157,
    pages = {167-176},
      doi = {10.1007/s11214-010-9699-y},
   adsurl = {http://adsabs.harvard.edu/abs/2010SSRv..157..167F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fabian2012,
   author = {{Fabian}, A.~C. and {Wilkins}, D.~R. and {Miller}, J.~M. and 
	{Reis}, R.~C. and {Reynolds}, C.~S. and {Cackett}, E.~M. and 
	{Nowak}, M.~A. and {Pooley}, G.~G. and {Pottschmidt}, K. and 
	{Sanders}, J.~S. and {Ross}, R.~R. and {Wilms}, J.},
    title = "{On the determination of the spin of the black hole in Cyg X-1 from X-ray reflection spectra}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1204.5854},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, black hole physics, line: profiles, X-rays: general},
     year = 2012,
    month = jul,
   volume = 424,
    pages = {217-223},
      doi = {10.1111/j.1365-2966.2012.21185.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.424..217F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fabian2015,
   author = {{Fabian}, A.~C. and {Lohfink}, A. and {Kara}, E. and {Parker}, M.~L. and 
	{Vasudevan}, R. and {Reynolds}, C.~S.},
    title = "{Properties of AGN coronae in the NuSTAR era}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1505.07603},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, black hole physics, X-rays: binaries, X-rays: galaxies},
     year = 2015,
    month = aug,
   volume = 451,
    pages = {4375-4383},
      doi = {10.1093/mnras/stv1218},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.451.4375F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gandhi2019,
   author = {{Gandhi}, P. and {Rao}, A. and {Johnson}, M.~A.~C. and {Paice}, J.~A. and 
	{Maccarone}, T.~J.},
    title = "{Gaia Data Release 2 distances and peculiar velocities for Galactic black hole transients}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1804.11349},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, parallaxes, proper motions, stars: black holes, stars: distances},
     year = 2019,
    month = may,
   volume = 485,
    pages = {2642-2655},
      doi = {10.1093/mnras/stz438},
   adsurl = {http://adsabs.harvard.edu/abs/2019MNRAS.485.2642G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garcia2010,
	author = {{Garc{\'{\i}}a}, J. and {Kallman}, T.~R.},
	title = "{X-ray Reflected Spectra from Accretion Disk Models. I. Constant Density Atmospheres}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1006.0485},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion disks, atomic processes, black hole physics, line: formation, radiative transfer, X-rays: general},
	year = 2010,
	month = aug,
	volume = 718,
	pages = {695-706},
	doi = {10.1088/0004-637X/718/2/695},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...718..695G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garcia2013,
	author = {{Garc{\'{\i}}a}, J. and {Dauser}, T. and {Reynolds}, C.~S. and 
	{Kallman}, T.~R. and {McClintock}, J.~E. and {Wilms}, J. and 
	{Eikmann}, W.},
	title = "{X-Ray Reflected Spectra from Accretion Disk Models. III. A Complete Grid of Ionized Reflection Calculations}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1303.2112},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion disks, atomic processes, black hole physics, line: formation, radiative transfer, X-rays: general },
	year = 2013,
	month = may,
	volume = 768,
	eid = {146},
	pages = {146},
	doi = {10.1088/0004-637X/768/2/146},
	adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...768..146G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garcia2013b,
	author = {{Garc{\'{\i}}a}, J. and {Elhoussieny}, E.~E. and {Bautista}, M.~A. and 
	{Kallman}, T.~R.},
	title = "{Time-dependent Photoionization of Gaseous Nebulae: The Pure Hydrogen Case}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1308.0258},
	primaryClass = "astro-ph.HE",
	keywords = {galaxies: nuclei, galaxies: Seyfert, H II regions, methods: numerical, planetary nebulae: general, plasmas, quasars: general },
	year = 2013,
	month = sep,
	volume = 775,
	eid = {8},
	pages = {8},
	doi = {10.1088/0004-637X/775/1/8},
	adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...775....8G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garcia2014,
   author = {{Garc{\'{\i}}a}, J. and {Dauser}, T. and {Lohfink}, A. and {Kallman}, T.~R. and 
	{Steiner}, J.~F. and {McClintock}, J.~E. and {Brenneman}, L. and 
	{Wilms}, J. and {Eikmann}, W. and {Reynolds}, C.~S. and {Tombesi}, F.
	},
    title = "{Improved Reflection Models of Black Hole Accretion Disks: Treating the Angular Distribution of X-Rays}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1312.3231},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, black hole physics, galaxies: individual: Ark 120, line: formation, radiative transfer, X-rays: general},
     year = 2014,
    month = feb,
   volume = 782,
      eid = {76},
    pages = {76},
      doi = {10.1088/0004-637X/782/2/76},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...782...76G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garcia2015,
	author = {{Garc{\'{\i}}a}, J.~A. and {Steiner}, J.~F. and {McClintock}, J.~E. and 
	{Remillard}, R.~A. and {Grinberg}, V. and {Dauser}, T.},
	title = "{X-Ray Reflection Spectroscopy of the Black Hole GX 339--4: Exploring the Hard State with Unprecedented Sensitivity}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1505.03607},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion disks, atomic processes, black hole physics, line: formation, X-rays: individual: GX 339{\ndash}4},
	year = 2015,
	month = nov,
	volume = 813,
	eid = {84},
	pages = {84},
	doi = {10.1088/0004-637X/813/2/84},
	adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...813...84G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garcia2016,
   author = {{Garc{\'{\i}}a}, J.~A. and {Fabian}, A.~C. and {Kallman}, T.~R. and 
	{Dauser}, T. and {Parker}, M.~L. and {McClintock}, J.~E. and 
	{Steiner}, J.~F. and {Wilms}, J.},
    title = "{The effects of high density on the X-ray spectrum reflected from accretion discs around black holes}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1603.05259},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, atomic processes, line: formation, radiative transfer, relativistic processes, X-rays: general},
     year = 2016,
    month = oct,
   volume = 462,
    pages = {751-760},
      doi = {10.1093/mnras/stw1696},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.462..751G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gardner2017,
       author = {{Gardner}, Emma and {Done}, Chris},
        title = "{The origin of the UV/optical lags in NGC 5548}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, galaxies: active, galaxies: individual: NGC 5548, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = sep,
       volume = {470},
       number = {3},
        pages = {3591-3605},
          doi = {10.1093/mnras/stx946},
archivePrefix = {arXiv},
       eprint = {1603.09564},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.3591G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{George1991,
   author = {{George}, I.~M. and {Fabian}, A.~C.},
    title = "{X-ray reflection from cold matter in active galactic nuclei and X-ray binaries}",
  journal = {\mnras},
 keywords = {Active Galactic Nuclei, Cold Plasmas, Computational Astrophysics, Dark Matter, X Ray Binaries, Abundance, Compton Effect, Fluorescence, Monte Carlo Method, X Ray Irradiation},
     year = 1991,
    month = mar,
   volume = 249,
    pages = {352-367},
      doi = {10.1093/mnras/249.2.352},
   adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.249..352G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gelman1992,
       author = {{Gelman}, Andrew and {Rubin}, Donald B.},
        title = "{Inference from Iterative Simulation Using Multiple Sequences}",
      journal = {Statistical Science},
         year = "1992",
        month = "Jan",
       volume = {7},
        pages = {457-472},
          doi = {10.1214/ss/1177011136},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992StaSc...7..457G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Geweke1992,
    author = {John Geweke},
    title = {Evaluating the Accuracy of Sampling-Based Approaches to the Calculation of Posterior Moments},
    booktitle = {IN BAYESIAN STATISTICS },
    year = {1992},
    pages = {169--193},
    publisher = {University Press}
}

@ARTICLE{Gilfanov2000,
	author = {{Gilfanov}, M. and {Churazov}, E. and {Revnivtsev}, M.},
	title = "{Frequency-resolved spectroscopy of Cyg X-1: fast variability of the reflected emission in the soft state}",
	journal = {\mnras},
	eprint = {astro-ph/0001450},
	keywords = {ACCRETION, ACCRETION DISCS, BLACK HOLE PHYSICS, BINARIES: GENERAL, STARS: INDIVIDUAL: CYG X-1, X-RAYS: GENERAL, X-RAYS: STARS},
	year = 2000,
	month = aug,
	volume = 316,
	pages = {923-928},
	doi = {10.1046/j.1365-8711.2000.03686.x},
	adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.316..923G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Grier2012,
       author = {{Grier}, C.~J. and {Peterson}, B.~M. and {Pogge}, R.~W. and
         {Denney}, K.~D. and {Bentz}, M.~C. and {Martini}, Paul and
         {Sergeev}, S.~G. and {Kaspi}, S. and {Zu}, Y. and {Kochanek}, C.~S. and
         {Shappee}, B.~J. and {Stanek}, K.~Z. and {Araya Salvo}, C. and
         {Beatty}, T.~G. and {Bird}, J.~C. and {Bord}, D.~J. and
         {Borman}, G.~A. and {Che}, X. and {Chen}, C. and {Cohen}, S.~A. and
         {Dietrich}, M. and {Doroshenko}, V.~T. and {Efimov}, Yu. S. and
         {Free}, N. and {Ginsburg}, I. and {Henderson}, C.~B. and
         {Horne}, Keith and {King}, A.~L. and {Mogren}, K. and {Molina}, M. and
         {Mosquera}, A.~M. and {Nazarov}, S.~V. and {Okhmat}, D.~N. and
         {Pejcha}, O. and {Rafter}, S. and {Shields}, J.~C. and {Skowron}, J. and
         {Szczygiel}, D.~M. and {Valluri}, M. and {van Saders}, J.~L.},
        title = "{A Reverberation Lag for the High-ionization Component of the Broad-line Region in the Narrow-line Seyfert 1 Mrk 335}",
      journal = {\apjl},
     keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Jan",
       volume = {744},
       number = {1},
          eid = {L4},
        pages = {L4},
          doi = {10.1088/2041-8205/744/1/L4},
archivePrefix = {arXiv},
       eprint = {1110.6179},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...744L...4G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Grinberg2014,
	author = {{Grinberg}, V. and {Pottschmidt}, K. and {B{\"o}ck}, M. and 
	{Schmid}, C. and {Nowak}, M.~A. and {Uttley}, P. and {Tomsick}, J.~A. and 
	{Rodriguez}, J. and {Hell}, N. and {Markowitz}, A. and {Bodaghee}, A. and 
	{Cadolle Bel}, M. and {Rothschild}, R.~E. and {Wilms}, J.},
	title = "{Long term variability of Cygnus X-1. VI. Energy-resolved X-ray variability 1999-2011}",
	journal = {\aap},
	archivePrefix = "arXiv",
	eprint = {1402.4485},
	primaryClass = "astro-ph.HE",
	keywords = {X-rays: binaries, stars: individual: Cygnus X-1, binaries: close},
	year = 2014,
	month = may,
	volume = 565,
	eid = {A1},
	pages = {A1},
	doi = {10.1051/0004-6361/201322969},
	adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...565A...1G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Grinberg2015,
	author = {{Grinberg}, V. and {Leutenegger}, M.~A. and {Hell}, N. and {Pottschmidt}, K. and 
	{B{\"o}ck}, M. and {Garc{\'{\i}}a}, J.~A. and {Hanke}, M. and 
	{Nowak}, M.~A. and {Sundqvist}, J.~O. and {Townsend}, R.~H.~D. and 
	{Wilms}, J.},
	title = "{Long term variability of Cygnus X-1. VII. Orbital variability of the focussed wind in Cyg X-1/HDE 226868 system}",
	journal = {\aap},
	archivePrefix = "arXiv",
	eprint = {1502.07343},
	primaryClass = "astro-ph.HE",
	keywords = {stars: individual: Cyg X-1, X-rays: binaries, binaries : close, stars: winds, outflows},
	year = 2015,
	month = apr,
	volume = 576,
	eid = {A117},
	pages = {A117},
	doi = {10.1051/0004-6361/201425418},
	adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...576A.117G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Grupe2007,
       author = {{Grupe}, Dirk and {Komossa}, Stefanie and {Gallo}, Luigi C.},
        title = "{Discovery of the Narrow-Line Seyfert 1 Galaxy Markarian 335 in a Historical Low X-Ray Flux State}",
      journal = {\apjl},
     keywords = {Galaxies: Active, Galaxies: Individual: Name: Markarian 335, Galaxies: Seyfert, Ultraviolet: Galaxies, X-Rays: Galaxies, Astrophysics},
         year = "2007",
        month = "Oct",
       volume = {668},
       number = {2},
        pages = {L111-L114},
          doi = {10.1086/523042},
archivePrefix = {arXiv},
       eprint = {0709.0733},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...668L.111G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Heil2015,
	author = {{Heil}, L.~M. and {Uttley}, P. and {Klein-Wolt}, M.},
	title = "{Inclination-dependent spectral and timing properties in transient black hole X-ray binaries}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1405.2026},
	primaryClass = "astro-ph.HE",
	keywords = {X-rays: binaries, X-rays: general},
	year = 2015,
	month = apr,
	volume = 448,
	pages = {3348-3353},
	doi = {10.1093/mnras/stv240},
	adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.448.3348H},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Huchra1999,
       author = {{Huchra}, John P. and {Vogeley}, Michael S. and {Geller}, Margaret J.},
        title = "{The CFA Redshift Survey: Data for the South Galactic CAP}",
      journal = {\apjs},
     keywords = {GALAXIES: DISTANCES AND REDSHIFTS, COSMOLOGY: LARGE-SCALE STRUCTURE OF UNIVERSE, SURVEYS, Galaxies: Distances and Redshifts, Cosmology: Large-Scale Structure of Universe, Surveys},
         year = "1999",
        month = "Apr",
       volume = {121},
       number = {2},
        pages = {287-368},
          doi = {10.1086/313194},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJS..121..287H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kalberla2005,
       author = {{Kalberla}, P.~M.~W. and {Burton}, W.~B. and {Hartmann}, Dap and
         {Arnal}, E.~M. and {Bajaja}, E. and {Morras}, R. and
         {P{\"o}ppel}, W.~G.~L.},
        title = "{The Leiden/Argentine/Bonn (LAB) Survey of Galactic HI. Final data release of the combined LDS and IAR surveys with improved stray-radiation corrections}",
      journal = {\aap},
     keywords = {surveys, radio lines: ISM, Galaxy: structure, Astrophysics},
         year = "2005",
        month = "Sep",
       volume = {440},
       number = {2},
        pages = {775-782},
          doi = {10.1051/0004-6361:20041864},
archivePrefix = {arXiv},
       eprint = {astro-ph/0504140},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...440..775K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kammoun2019,
   author = {{Kammoun}, E.~S. and {Dom{\v c}ek}, V. and {Svoboda}, J. and 
	{Dov{\v c}iak}, M. and {Matt}, G.},
    title = "{Steep X-ray reflection emissivity profiles in AGN as the result of radially structured disc ionization}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1902.03481},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, black hole physics, relativistic processes, galaxies: nuclei, X-rays: galaxies},
     year = 2019,
    month = may,
   volume = 485,
    pages = {239-247},
      doi = {10.1093/mnras/stz408},
   adsurl = {http://adsabs.harvard.edu/abs/2019MNRAS.485..239K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kara2013a,
	author = {{Kara}, E. and {Fabian}, A.~C. and {Cackett}, E.~M. and {Steiner}, J.~F. and 
	{Uttley}, P. and {Wilkins}, D.~R. and {Zoghbi}, A.},
	title = "{The closest look at 1H0707-495: X-ray reverberation lags with 1.3 Ms of data}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1210.1465},
	primaryClass = "astro-ph.HE",
	keywords = {black hole physics, galaxies: active, X-rays: galaxies},
	year = 2013,
	month = feb,
	volume = 428,
	pages = {2795-2804},
	doi = {10.1093/mnras/sts155},
	adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.428.2795K},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kara2013b,
	author = {{Kara}, E. and {Fabian}, A.~C. and {Cackett}, E.~M. and {Uttley}, P. and 
	{Wilkins}, D.~R. and {Zoghbi}, A.},
	title = "{Discovery of high-frequency iron K lags in Ark 564 and Mrk 335}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1306.2551},
	primaryClass = "astro-ph.HE",
	keywords = {black hole physics, galaxies: active, X-rays: galaxies},
	year = 2013,
	month = sep,
	volume = 434,
	pages = {1129-1137},
	doi = {10.1093/mnras/stt1055},
	adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.434.1129K},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kara2013c,
	author = {{Kara}, E. and {Fabian}, A.~C. and {Cackett}, E.~M. and {Miniutti}, G. and 
	{Uttley}, P.},
	title = "{Revealing the X-ray source in IRAS 13224-3809 through flux-dependent reverberation lags}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1301.1924},
	primaryClass = "astro-ph.HE",
	keywords = {black hole physics, galaxies: active, X-rays: galaxies},
	year = 2013,
	month = apr,
	volume = 430,
	pages = {1408-1413},
	doi = {10.1093/mnras/stt024},
	adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.430.1408K},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kara2016,
	author = {{Kara}, E. and {Alston}, W.~N. and {Fabian}, A.~C. and {Cackett}, E.~M. and 
	{Uttley}, P. and {Reynolds}, C.~S. and {Zoghbi}, A.},
	title = "{A global look at X-ray time lags in Seyfert galaxies}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1605.02631},
	primaryClass = "astro-ph.HE",
	keywords = {black hole physics, galaxies: active, X-rays: galaxies},
	year = 2016,
	month = oct,
	volume = 462,
	pages = {511-531},
	doi = {10.1093/mnras/stw1695},
	adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.462..511K},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kara2019,
   author = {{Kara}, E. and {Steiner}, J.~F. and {Fabian}, A.~C. and {Cackett}, E.~M. and 
	{Uttley}, P. and {Remillard}, R.~A. and {Gendreau}, K.~C. and 
	{Arzoumanian}, Z. and {Altamirano}, D. and {Eikenberry}, S. and 
	{Enoto}, T. and {Homan}, J. and {Neilsen}, J. and {Stevens}, A.~L.
	},
    title = "{The corona contracts in a black-hole transient}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1901.03877},
 primaryClass = "astro-ph.HE",
     year = 2019,
    month = jan,
   volume = 565,
    pages = {198-201},
      doi = {10.1038/s41586-018-0803-x},
   adsurl = {http://adsabs.harvard.edu/abs/2019Natur.565..198K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Keek2016,
       author = {{Keek}, L. and {Ballantyne}, D.~R.},
        title = "{Revealing the accretion disc corona in Mrk 335 with multi-epoch X-ray spectroscopy}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, galaxies: active, galaxies: individual: Mrk 335, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2016",
        month = "Mar",
       volume = {456},
       number = {3},
        pages = {2722-2734},
          doi = {10.1093/mnras/stv2882},
archivePrefix = {arXiv},
       eprint = {1508.06994},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.456.2722K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Klis1987,
	author = {{van der Klis}, M. and {Hasinger}, G. and {Stella}, L. and {Langmeier}, A. and 
	{van Paradijs}, J. and {Lewin}, W.~H.~G.},
	title = "{The complex cross-spectra of Cygnus X-2 and GX 5-1}",
	journal = {\apjl},
	keywords = {Radiant Flux Density, Stellar Oscillations, Stellar Spectra, X Ray Binaries, Time Lag, Vibrational Spectra},
	year = 1987,
	month = aug,
	volume = 319,
	pages = {L13-L18},
	doi = {10.1086/184946},
	adsurl = {http://adsabs.harvard.edu/abs/1987ApJ...319L..13V},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kording2004,
	author = {{K{\"o}rding}, E. and {Falcke}, H.},
	title = "{X-ray time lags from a pivoting power law in black holes}",
	journal = {\aap},
	eprint = {astro-ph/0310641},
	keywords = {X-rays: binaries, accretion, accretion disks, black hole physics, radiation mechanisms: non-thermal},
	year = 2004,
	month = feb,
	volume = 414,
	pages = {795-806},
	doi = {10.1051/0004-6361:20031614},
	adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...414..795K},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kotov2001,
	author = {{Kotov}, O. and {Churazov}, E. and {Gilfanov}, M.},
	title = "{On the X-ray time-lags in the black hole candidates}",
	journal = {\mnras},
	eprint = {astro-ph/0103115},
	keywords = {ACCRETION, ACCRETION DISCS, STARS: INDIVIDUAL: CYGNUS X-1, X-RAYS: GENERAL, X-RAYS: STARS},
	year = 2001,
	month = nov,
	volume = 327,
	pages = {799-807},
	doi = {10.1046/j.1365-8711.2001.04769.x},
	adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.327..799K},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ingram2009,
	author = {{Ingram}, A. and {Done}, C. and {Fragile}, P.~C.},
	title = "{Low-frequency quasi-periodic oscillations spectra and Lense-Thirring precession}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {0901.1238},
	primaryClass = "astro-ph.SR",
	keywords = {accretion, accretion discs, black hole physics, X-rays: binaries},
	year = 2009,
	month = jul,
	volume = 397,
	pages = {L101-L105},
	doi = {10.1111/j.1745-3933.2009.00693.x},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.397L.101I},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ingram2013,
	author = {{Ingram}, A. and {van der Klis}, M.},
	title = "{An exact analytic treatment of propagating mass accretion rate fluctuations in X-ray binaries}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1306.3823},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, X-rays: binaries},
	year = 2013,
	month = sep,
	volume = 434,
	pages = {1476-1485},
	doi = {10.1093/mnras/stt1107},
	adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.434.1476I},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ingram2015,
	author = {{Ingram}, A. and {Maccarone}, T.~J. and {Poutanen}, J. and {Krawczynski}, H.
	},
	title = "{Polarization Modulation from Lense{\ndash}Thirring Precession in X-Ray Binaries}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1505.00015},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion disks, black hole physics, polarization, X-rays: binaries},
	year = 2015,
	month = jul,
	volume = 807,
	eid = {53},
	pages = {53},
	doi = {10.1088/0004-637X/807/1/53},
	adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...807...53I},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ingram2016,
	author = {{Ingram}, A. and {van der Klis}, M. and {Middleton}, M. and 
	{Done}, C. and {Altamirano}, D. and {Heil}, L. and {Uttley}, P. and 
	{Axelsson}, M.},
	title = "{A quasi-periodic modulation of the iron line centroid energy in the black hole binary H1743-322}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1607.02866},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, black hole physics, relativistic processes, X-rays: individual: H1743-322},
	year = 2016,
	month = sep,
	volume = 461,
	pages = {1967-1980},
	doi = {10.1093/mnras/stw1245},
	adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.461.1967I},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ingram2017,
	author = {{Ingram}, A. and {van der Klis}, M. and {Middleton}, M. and 
	{Altamirano}, D. and {Uttley}, P.},
	title = "{Tomographic reflection modelling of quasi-periodic oscillations in the black hole binary H 1743-322}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1610.00948},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, black hole physics, X-rays: individual: H 1743-322},
	year = 2017,
	month = jan,
	volume = 464,
	pages = {2979-2991},
	doi = {10.1093/mnras/stw2581},
	adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.464.2979I},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ingram2019,
       author = {{Ingram}, Adam and {Mastroserio}, Guglielmo and {Dauser}, Thomas and
         {Hovenkamp}, Pieter and {van der Klis}, Michiel and
         {Garc{\'\i}a}, Javier A.},
        title = "{A public relativistic transfer function model for X-ray reverberation mapping of accreting black holes}",
      journal = {\mnras},
     keywords = {black hole physics, methods: data analysis, galaxies: active, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Jun",
        pages = {1677},
          doi = {10.1093/mnras/stz1720},
archivePrefix = {arXiv},
       eprint = {1906.08310},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.tmp.1677I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Longinotti2013,
       author = {{Longinotti}, A.~L. and {Krongold}, Y. and {Kriss}, G.~A. and {Ely}, J. and
         {Gallo}, L. and {Grupe}, D. and {Komossa}, S. and {Mathur}, S. and
         {Pradhan}, A.},
        title = "{The Rise of an Ionized Wind in the Narrow-line Seyfert 1 Galaxy Mrk 335 Observed by XMM-Newton and HST}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: Seyfert, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2013",
        month = "Apr",
       volume = {766},
       number = {2},
          eid = {104},
        pages = {104},
          doi = {10.1088/0004-637X/766/2/104},
archivePrefix = {arXiv},
       eprint = {1301.5463},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...766..104L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lyubarskii1997,
	author = {{Lyubarskii}, Y.~E.},
	title = "{Flicker noise in accretion discs}",
	journal = {\mnras},
	keywords = {Accretion Disks, Noise Measurement, Mass Transfer, Luminosity, X Ray Sources, Computational Astrophysics, Radial Distribution},
	year = 1997,
	month = dec,
	volume = 292,
	pages = {679},
	doi = {10.1093/mnras/292.3.679},
	adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.292..679L},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Luminet1979,
	author = {{Luminet}, J.-P.},
	title = "{Image of a spherical black hole with thin accretion disk}",
	journal = {\aap},
	keywords = {Black Holes (Astronomy), Stellar Mass Accretion, Doppler Effect, Optics, Radiation Distribution, Spheres},
	year = 1979,
	month = may,
	volume = 75,
	pages = {228-235},
	adsurl = {http://adsabs.harvard.edu/abs/1979A%26A....75..228L},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mahmoud2018a,
   author = {{Mahmoud}, R.~D. and {Done}, C.},
    title = "{Modelling the energy dependence of black hole binary flows}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1706.05357},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual: Cygnus X-1},
     year = 2018,
    month = jan,
   volume = 473,
    pages = {2084-2097},
      doi = {10.1093/mnras/stx2359},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.473.2084M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mahmoud2018b,
   author = {{Mahmoud}, R.~D. and {Done}, C.},
    title = "{A physical model for the spectral-timing properties of accreting black holes}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1803.04811},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual: Cygnus X-1},
     year = 2018,
    month = nov,
   volume = 480,
    pages = {4040-4059},
      doi = {10.1093/mnras/sty2133},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.480.4040M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mahmoud2019,
   author = {{Mahmoud}, R.~D. and {Done}, C. and {De Marco}, B.},
    title = "{Reverberation Reveals the Truncated Disc in the Hard State of GX 339-4}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1811.06911},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena},
     year = 2018,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv181106911M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Markoff2005,
   author = {{Markoff}, S. and {Nowak}, M.~A. and {Wilms}, J.},
    title = "{Going with the Flow: Can the Base of Jets Subsume the Role of Compact Accretion Disk Coronae?}",
  journal = {\apj},
   eprint = {astro-ph/0509028},
 keywords = {Accretion, Accretion Disks, Black Hole Physics, Radiation Mechanisms: Nonthermal, X-Rays: Binaries, X-Rays: General},
     year = 2005,
    month = dec,
   volume = 635,
    pages = {1203-1216},
      doi = {10.1086/497628},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...635.1203M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Martocchia2000,
   author = {{Martocchia}, A. and {Karas}, V. and {Matt}, G.},
    title = "{Effects of Kerr space-time on spectral features from X-ray illuminated accretion discs}",
  journal = {\mnras},
   eprint = {astro-ph/9910562},
 keywords = {ACCRETION, ACCRETION DISCS, BLACK HOLE PHYSICS, LINE: FORMATION, RELATIVITY, GALAXIES: ACTIVE, X-RAYS: GALAXIES},
     year = 2000,
    month = mar,
   volume = 312,
    pages = {817-826},
      doi = {10.1046/j.1365-8711.2000.03205.x},
   adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.312..817M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mastroserio2018,
   author = {{Mastroserio}, G. and {Ingram}, A. and {van der Klis}, M.},
    title = "{Multi-time-scale X-ray reverberation mapping of accreting black holes}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1801.03100},
 primaryClass = "astro-ph.HE",
 keywords = {black hole physics, methods: data analysis, galaxies: active, X-rays: binaries},
     year = 2018,
    month = apr,
   volume = 475,
    pages = {4027-4042},
      doi = {10.1093/mnras/sty075},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.475.4027M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mastroserio2019,
       author = {{Mastroserio}, Guglielmo and {Ingram}, Adam and {van der Klis}, Michiel},
        title = "{An X-ray reverberation mass measurement of Cygnus X-1}",
      journal = {\mnras},
     keywords = {black hole physics, relativistic processes, methods: data analysis, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Jun",
        pages = {1682},
          doi = {10.1093/mnras/stz1727},
archivePrefix = {arXiv},
       eprint = {1906.08266},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.tmp.1682M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Matt1991,
	author = {{Matt}, G. and {Perola}, G.~C. and {Piro}, L.},
	title = "{The iron line and high energy bump as X-ray signatures of cold matter in Seyfert 1 galaxies}",
	journal = {\aap},
	keywords = {Galactic Radiation, Seyfert Galaxies, X Ray Spectra, Black Holes (Astronomy), Iron, Line Spectra},
	year = 1991,
	month = jul,
	volume = 247,
	pages = {25-34},
	adsurl = {http://adsabs.harvard.edu/abs/1991A%26A...247...25M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Matt1992,
	author = {{Matt}, G. and {Perola}, G.~C. and {Piro}, L. and {Stella}, L.
	},
	title = "{Iron K-alpha line from X-ray illuminated relativistic disks}",
	journal = {\aap},
	keywords = {Accretion Disks, Iron, K Lines, X Ray Sources, Astronomical Models, Emission Spectra, Fluorescence, Seyfert Galaxies, Spectral Line Width},
	year = 1992,
	month = apr,
	volume = 257,
	pages = {63-68},
	adsurl = {http://adsabs.harvard.edu/abs/1992A%26A...257...63M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McHardy2004,
	author = {{McHardy}, I.~M. and {Papadakis}, I.~E. and {Uttley}, P. and 
	{Page}, M.~J. and {Mason}, K.~O.},
	title = "{Combined long and short time-scale X-ray variability of NGC 4051 with RXTE and XMM-Newton}",
	journal = {\mnras},
	eprint = {astro-ph/0311220},
	keywords = {black hole physics, galaxies: active, galaxies: individual: NGC 4051, X-rays: binaries, X-rays: galaxies},
	year = 2004,
	month = mar,
	volume = 348,
	pages = {783-801},
	doi = {10.1111/j.1365-2966.2004.07376.x},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.348..783M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Miller2010,
	author = {{Miller}, L. and {Turner}, T.~J. and {Reeves}, J.~N. and {Braito}, V.
	},
	title = "{X-ray reverberation in 1H0707-495 revisited}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1006.5035},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, galaxies: active, galaxies: individual: 1H0707-495, X-rays: galaxies},
	year = 2010,
	month = nov,
	volume = 408,
	pages = {1928-1935},
	doi = {10.1111/j.1365-2966.2010.17261.x},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.408.1928M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mirabel2003,
   author = {{Mirabel}, I.~F. and {Rodrigues}, I.},
    title = "{Formation of a Black Hole in the Dark}",
  journal = {Science},
   eprint = {astro-ph/0305205},
     year = 2003,
    month = may,
   volume = 300,
    pages = {1119-1121},
      doi = {10.1126/science.1083451},
   adsurl = {http://adsabs.harvard.edu/abs/2003Sci...300.1119M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Misra2013,
	author = {{Misra}, R. and {Mandal}, S.},
	title = "{Alternating Lags of QPO Harmonics: A Generic Model and its Application to the 67 mHz QPO of GRS 1915+105}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1310.4338},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion disks, black hole physics, stars: individual: GRS 1915+105 },
	year = 2013,
	month = dec,
	volume = 779,
	eid = {71},
	pages = {71},
	doi = {10.1088/0004-637X/779/1/71},
	adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...779...71M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mitsuda1989,
	author = {{Mitsuda}, K. and {Dotani}, T.},
	title = "{Energy-dependent time lags in QPO from Cygnus X-2}",
	journal = {\pasj},
	keywords = {Cygnus Constellation, Neutron Stars, Stellar Oscillations, Time Lag, X Ray Binaries, Japanese Space Program, Phase Shift, Satellite Observation},
	year = 1989,
	volume = 41,
	pages = {557-575},
	adsurl = {http://adsabs.harvard.edu/abs/1989PASJ...41..557M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Miyamoto1988,
	author = {{Miyamoto}, S. and {Kitamoto}, S. and {Mitsuda}, K. and {Dotani}, T.
	},
	title = "{Delayed hard X-rays from Cygnus X-1}",
	journal = {\nat},
	keywords = {Black Holes (Astronomy), Cygnus Constellation, X Ray Sources, X Ray Spectra, Compton Effect, Cross Correlation, Delay},
	year = 1988,
	month = dec,
	volume = 336,
	pages = {450-452},
	doi = {10.1038/336450a0},
	adsurl = {http://adsabs.harvard.edu/abs/1988Natur.336..450M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Miyamoto1989,
	author = {{Miyamoto}, S. and {Kitamoto}, S.},
	title = "{X-ray time variations from Cygnus X-1 and implications for the accretion process}",
	journal = {\nat},
	keywords = {Gravitational Effects, Spectrum Analysis, Stellar Mass Accretion, Time Lag, X Ray Sources, Black Holes (Astronomy), Companion Stars, Cygnus Constellation, O Stars, X Ray Spectra},
	year = 1989,
	month = dec,
	volume = 342,
	pages = {773},
	doi = {10.1038/342773a0},
	adsurl = {http://adsabs.harvard.edu/abs/1989Natur.342..773M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mizumoto2018,
   author = {{Mizumoto}, M. and {Done}, C. and {Hagino}, K. and {Ebisawa}, K. and 
	{Tsujimoto}, M. and {Odaka}, H.},
    title = "{X-ray short-time lags in the Fe-K energy band produced by scattering clouds in active galactic nuclei}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1805.00046},
 primaryClass = "astro-ph.HE",
 keywords = {black hole physics, galaxies: active, galaxies: Seyfert, X-rays: galaxies},
     year = 2018,
    month = jul,
   volume = 478,
    pages = {971-982},
      doi = {10.1093/mnras/sty1114},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.478..971M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Motta2015,
	author = {{Motta}, S.~E. and {Casella}, P. and {Henze}, M. and {Mu{\~n}oz-Darias}, T. and 
	{Sanna}, A. and {Fender}, R. and {Belloni}, T.},
	title = "{Geometrical constraints on the origin of timing signals from black holes}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1404.7293},
	primaryClass = "astro-ph.HE",
	keywords = {binaries: close, stars: black holes, stars: jets, stars: low-mass, stars: oscillations, X-rays: binaries},
	year = 2015,
	month = feb,
	volume = 447,
	pages = {2059-2072},
	doi = {10.1093/mnras/stu2579},
	adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.447.2059M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Niedzwiecki2016,
	author = {{Nied{\'z}wiecki}, A. and {Zdziarski}, A.~A. and {Szanecki}, M.
	},
	title = "{On the Lamppost Model of Accreting Black Holes}",
	journal = {\apjl},
	archivePrefix = "arXiv",
	eprint = {1602.09075},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion disks, black hole physics, galaxies: active, galaxies: individual: NGC 4151, stars: individual: Cyg X-1, X-rays: binaries},
	year = 2016,
	month = apr,
	volume = 821,
	eid = {L1},
	pages = {L1},
	doi = {10.3847/2041-8205/821/1/L1},
	adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...821L...1N},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nowak1999,
	author = {{Nowak}, M.~A. and {Vaughan}, B.~A. and {Wilms}, J. and {Dove}, J.~B. and 
	{Begelman}, M.~C.},
	title = "{Rossi X-Ray Timing Explorer Observation of Cygnus X-1. II. Timing Analysis}",
	journal = {\apj},
	keywords = {ACCRETION, ACCRETION DISKS, BLACK HOLE PHYSICS, STARS: INDIVIDUAL: CONSTELLATION NAME: CYGNUS X-1, X-RAYS: STARS, Accretion, Accretion Disks, Black Hole Physics, Stars: Individual: Constellation Name: Cygnus X-1, X-Rays: Stars},
	year = 1999,
	month = jan,
	volume = 510,
	pages = {874-891},
	doi = {10.1086/306610},
	adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...510..874N},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Onken2004,
       author = {{Onken}, Christopher A. and {Ferrarese}, Laura and {Merritt}, David and
         {Peterson}, Bradley M. and {Pogge}, Richard W. and
         {Vestergaard}, Marianne and {Wandel}, Amri},
        title = "{Supermassive Black Holes in Active Galactic Nuclei. II. Calibration of the Black Hole Mass-Velocity Dispersion Relationship for Active Galactic Nuclei}",
      journal = {\apj},
     keywords = {Black Hole Physics, Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Astrophysics},
         year = 2004,
        month = nov,
       volume = {615},
       number = {2},
        pages = {645-651},
          doi = {10.1086/424655},
archivePrefix = {arXiv},
       eprint = {astro-ph/0407297},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...615..645O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Orosz2011,
	author = {{Orosz}, J.~A. and {McClintock}, J.~E. and {Aufdenberg}, J.~P. and 
	{Remillard}, R.~A. and {Reid}, M.~J. and {Narayan}, R. and {Gou}, L.
	},
	title = "{The Mass of the Black Hole in Cygnus X-1}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1106.3689},
	primaryClass = "astro-ph.HE",
	keywords = {binaries: general, black hole physics, stars: individual: Cygnus X-1, X-rays: binaries},
	year = 2011,
	month = dec,
	volume = 742,
	eid = {84},
	pages = {84},
	doi = {10.1088/0004-637X/742/2/84},
	adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...742...84O},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Page2004,
	author = {{Page}, K.~L. and {Schartel}, N. and {Turner}, M.~J.~L. and 
	{O'Brien}, P.~T.},
	title = "{XMM-Newton observations of seven soft X-ray excess quasi-stellar objects}",
	journal = {\mnras},
	eprint = {astro-ph/0404444},
	keywords = {galaxies: active, quasars: general, X-rays: galaxies},
	year = 2004,
	month = aug,
	volume = 352,
	pages = {523-534},
	doi = {10.1111/j.1365-2966.2004.07939.x},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.352..523P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Papadakis2001,
	author = {{Papadakis}, I.~E. and {Nandra}, K. and {Kazanas}, D.},
	title = "{Frequency-dependent Time Lags in the X-Ray Emission of the Seyfert Galaxy NGC 7469}",
	journal = {\apjl},
	eprint = {astro-ph/0106175},
	keywords = {Galaxies: Active, Galaxies: Individual: NGC Number: NGC 7469, Galaxies: Nuclei, X-Rays: Galaxies},
	year = 2001,
	month = jun,
	volume = 554,
	pages = {L133-L137},
	doi = {10.1086/321722},
	adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...554L.133P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parker2015,
	author = {{Parker}, M.~L. and {Tomsick}, J.~A. and {Miller}, J.~M. and 
	{Yamaoka}, K. and {Lohfink}, A. and {Nowak}, M. and {Fabian}, A.~C. and 
	{Alston}, W.~N. and {Boggs}, S.~E. and {Christensen}, F.~E. and 
	{Craig}, W.~W. and {F{\"u}rst}, F. and {Gandhi}, P. and {Grefenstette}, B.~W. and 
	{Grinberg}, V. and {Hailey}, C.~J. and {Harrison}, F.~A. and 
	{Kara}, E. and {King}, A.~L. and {Stern}, D. and {Walton}, D.~J. and 
	{Wilms}, J. and {Zhang}, W.~W.},
	title = "{NuSTAR and Suzaku Observations of the Hard State in Cygnus X-1: Locating the Inner Accretion Disk}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1506.00007},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion disks, black hole physics, X-rays: binaries, X-rays: individual: Cygnus X-1},
	year = 2015,
	month = jul,
	volume = 808,
	eid = {9},
	pages = {9},
	doi = {10.1088/0004-637X/808/1/9},
	adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...808....9P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parker2016,
   author = {{Parker}, M.~L. and {Tomsick}, J.~A. and {Kennea}, J.~A. and 
	{Miller}, J.~M. and {Harrison}, F.~A. and {Barret}, D. and {Boggs}, S.~E. and 
	{Christensen}, F.~E. and {Craig}, W.~W. and {Fabian}, A.~C. and 
	{F{\"u}rst}, F. and {Grinberg}, V. and {Hailey}, C.~J. and {Romano}, P. and 
	{Stern}, D. and {Walton}, D.~J. and {Zhang}, W.~W.},
    title = "{NuSTAR and Swift Observations of the Very High State in GX 339-4: Weighing the Black Hole with X-Rays}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1603.03777},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, X-rays: binaries, X-rays: individual: GX 339-4},
     year = 2016,
    month = apr,
   volume = 821,
      eid = {L6},
    pages = {L6},
      doi = {10.3847/2041-8205/821/1/L6},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...821L...6P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Peterson1993,
       author = {{Peterson}, Bradley M.},
        title = "{Reverberation Mapping of Active Galactic Nuclei}",
      journal = {\pasp},
     keywords = {Active Galactic Nuclei, Astronomical Maps, Emission Spectra, Reverberation, Astronomical Spectroscopy, Cross Correlation, Luminosity, Spectral Line Width, Transfer Functions, Astrophysics, GALAXIES: ACTIVE, GALAXIES: NUCLEI, METHODS: ANALYTICAL},
         year = 1993,
        month = mar,
       volume = {105},
        pages = {247},
          doi = {10.1086/133140},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993PASP..105..247P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Peterson2004,
       author = {{Peterson}, B.~M. and {Ferrarese}, L. and {Gilbert}, K.~M. and
         {Kaspi}, S. and {Malkan}, M.~A. and {Maoz}, D. and {Merritt}, D. and
         {Netzer}, H. and {Onken}, C.~A. and {Pogge}, R.~W. and
         {Vestergaard}, M. and {Wandel}, A.},
        title = "{Central Masses and Broad-Line Region Sizes of Active Galactic Nuclei. II. A Homogeneous Analysis of a Large Reverberation-Mapping Database}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Quasars: Emission Lines, Astrophysics},
         year = "2004",
        month = "Oct",
       volume = {613},
       number = {2},
        pages = {682-699},
          doi = {10.1086/423269},
archivePrefix = {arXiv},
       eprint = {astro-ph/0407299},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...613..682P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Poutanen1999,
	author = {{Poutanen}, J. and {Fabian}, A.~C.},
	title = "{Spectral evolution of magnetic flares and time lags in accreting black hole sources}",
	journal = {\mnras},
	eprint = {astro-ph/9811306},
	year = 1999,
	month = jul,
	volume = 306,
	pages = {L31-L37},
	doi = {10.1046/j.1365-8711.1999.02735.x},
	adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.306L..31P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Poutanen2002,
	author = {{Poutanen}, J.},
	title = "{Impact of reverberation in flared accretion discs on temporal characteristics of X-ray binaries}",
	journal = {\mnras},
	eprint = {astro-ph/0106189},
	keywords = {accretion, accretion discs, black hole physics, methods: numerical, stars: individual: Cygnus X-1, X-rays: binaries},
	year = 2002,
	month = may,
	volume = 332,
	pages = {257-270},
	doi = {10.1046/j.1365-8711.2002.05272.x},
	adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.332..257P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rapisarda2016,
   author = {{Rapisarda}, S. and {Ingram}, A. and {Kalamkar}, M. and {van der Klis}, M.
	},
    title = "{Modelling the cross-spectral variability of the black hole binary MAXI J1659-152 with propagating accretion rate fluctuations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1607.08178},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual: (MAXI J1659-152)},
     year = 2016,
    month = nov,
   volume = 462,
    pages = {4078-4093},
      doi = {10.1093/mnras/stw1878},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.462.4078R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Rapisarda2017a,
   author = {{Rapisarda}, S. and {Ingram}, A. and {van der Klis}, M.},
    title = "{Cross-spectral modelling of the black hole X-ray binary XTE J1550-564: challenges to the propagating fluctuations paradigm}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1704.07705},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual: XTE J1550-564},
     year = 2017,
    month = aug,
   volume = 469,
    pages = {2011-2023},
      doi = {10.1093/mnras/stx991},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.469.2011R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rapisarda2017b,
   author = {{Rapisarda}, S. and {Ingram}, A. and {van der Klis}, M.},
    title = "{Modelling hard and soft states of Cygnus X-1 with propagating mass accretion rate fluctuations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1708.04182},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual (Cygnus X-1)},
     year = 2017,
    month = dec,
   volume = 472,
    pages = {3821-3832},
      doi = {10.1093/mnras/stx2110},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.472.3821R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Reid2011,
   author = {{Reid}, M.~J. and {McClintock}, J.~E. and {Narayan}, R. and 
	{Gou}, L. and {Remillard}, R.~A. and {Orosz}, J.~A.},
    title = "{The Trigonometric Parallax of Cygnus X-1}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.3688},
 primaryClass = "astro-ph.HE",
 keywords = {astrometry, black hole physics, stars: distances, stars: individual: Cygnus X-1, X-rays: binaries},
     year = 2011,
    month = dec,
   volume = 742,
      eid = {83},
    pages = {83},
      doi = {10.1088/0004-637X/742/2/83},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...742...83R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reynolds1999,
	author = {{Reynolds}, C.~S. and {Young}, A.~J. and {Begelman}, M.~C. and 
	{Fabian}, A.~C.},
	title = "{X-Ray Iron Line Reverberation from Black Hole Accretion Disks}",
	journal = {\apj},
	eprint = {astro-ph/9806327},
	keywords = {ACCRETION, ACCRETION DISKS, BLACK HOLE PHYSICS, GALAXIES: ACTIVE, GALAXIES: SEYFERT, X-RAYS: GALAXIES, Accretion, Accretion Disks, Black Hole Physics, galaxies: active, galaxies: Seyfert, X-rays: galaxies},
	year = 1999,
	month = mar,
	volume = 514,
	pages = {164-179},
	doi = {10.1086/306913},
	adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...514..164R},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Revnivtsev1999,
	author = {{Revnivtsev}, M. and {Gilfanov}, M. and {Churazov}, E.},
	title = "{The frequency resolved spectroscopy of CYG X-1: fast variability of the Fe K\_{$\alpha$} line}",
	journal = {\aap},
	eprint = {astro-ph/9906198},
	keywords = {METHODS: DATA ANALYSIS, STARS: BINARIES: GENERAL, STARS: INDIVIDUAL: (CYG X-1), X-RAYS: GENERAL},
	year = 1999,
	month = jul,
	volume = 347,
	pages = {L23-L26},
	adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...347L..23R},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ross2005,
   author = {{Ross}, R.~R. and {Fabian}, A.~C.},
    title = "{A comprehensive range of X-ray ionized-reflection models}",
  journal = {\mnras},
   eprint = {astro-ph/0501116},
 keywords = {accretion, accretion discs, line: formation, radiative transfer, galaxies: active, X-rays: general},
     year = 2005,
    month = mar,
   volume = 358,
    pages = {211-216},
      doi = {10.1111/j.1365-2966.2005.08797.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.358..211R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shaposhnikov2012,
	author = {{Shaposhnikov}, N.},
	title = "{On the Nature of Quasi-periodic Oscillation Phase Lags in Black Hole Candidates}",
	journal = {\apjl},
	archivePrefix = "arXiv",
	eprint = {1205.0748},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion disks, black hole physics, stars: individual: XTE J1550{\ndash}564, X-rays: binaries},
	year = 2012,
	month = jun,
	volume = 752,
	eid = {L25},
	pages = {L25},
	doi = {10.1088/2041-8205/752/2/L25},
	adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...752L..25S},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shakura1973,
	author = {{Shakura}, N.~I. and {Sunyaev}, R.~A.},
	title = "{Black holes in binary systems. Observational appearance.}",
	journal = {\aap},
	year = 1973,
	volume = 24,
	pages = {337-355},
	adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....24..337S},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shreeram2020,
       author = {{Shreeram}, Soumya and {Ingram}, Adam},
        title = "{Exploring the radial disc ionization profile of the black hole X-ray binary GRS 1915+105}",
      journal = {\mnras},
     keywords = {black hole physics, X-rays: binaries, X-rays: individual: GRS 1915+105, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = feb,
       volume = {492},
       number = {1},
        pages = {405-412},
          doi = {10.1093/mnras/stz3455},
archivePrefix = {arXiv},
       eprint = {1912.06833},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.492..405S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Silva2016,
       author = {{Silva}, C.~V. and {Uttley}, P. and {Costantini}, E.},
        title = "{Timing the warm absorber in NGC 4051}",
      journal = {\aap},
     keywords = {methods: data analysis, black hole physics, galaxies: Seyfert, galaxies: individual: NGC 4051, quasars: absorption lines, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Dec",
       volume = {596},
          eid = {A79},
        pages = {A79},
          doi = {10.1051/0004-6361/201628555},
archivePrefix = {arXiv},
       eprint = {1607.01065},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...596A..79S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stella1990,
   author = {{Stella}, L.},
    title = "{Measuring black hole mass through variable line profiles from accretion disks}",
  journal = {\nat},
 keywords = {Accretion Disks, Black Holes (Astronomy), Line Shape, Stellar Mass, Stellar Spectra, X Ray Spectra, Active Galactic Nuclei, Compton Effect, Emission Spectra, Red Shift, Schwarzschild Metric},
     year = 1990,
    month = apr,
   volume = 344,
    pages = {747-749},
      doi = {10.1038/344747a0},
   adsurl = {http://adsabs.harvard.edu/abs/1990Natur.344..747S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Svensson1984,
   author = {{Svensson}, R.},
    title = "{Steady mildly relativistic thermal plasmas - Processes and properties}",
  journal = {\mnras},
 keywords = {Cosmic Plasma, Plasma Clouds, Relativistic Plasmas, Thermal Plasmas, Bremsstrahlung, Electron-Positron Pairs, Luminosity, Pair Production, Photons, Steady State, Thermodynamic Equilibrium},
     year = 1984,
    month = jul,
   volume = 209,
    pages = {175-208},
      doi = {10.1093/mnras/209.2.175},
   adsurl = {http://adsabs.harvard.edu/abs/1984MNRAS.209..175S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Svensson1994,
   author = {{Svensson}, R. and {Zdziarski}, A.~A.},
    title = "{Black hole accretion disks with coronae}",
  journal = {\apj},
 keywords = {Accretion Disks, Active Galactic Nuclei, Black Holes (Astronomy), Stellar Coronas, Stellar Mass Accretion, Ultraviolet Spectra, X Ray Spectra, Mathematical Models, Stellar Models, Ultraviolet Astronomy, X Ray Astronomy},
     year = 1994,
    month = dec,
   volume = 436,
    pages = {599-606},
      doi = {10.1086/174934},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...436..599S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Svoboda2012,
   author = {{Svoboda}, J. and {Dov{\v c}iak}, M. and {Goosmann}, R.~W. and 
	{Jethwa}, P. and {Karas}, V. and {Miniutti}, G. and {Guainazzi}, M.
	},
    title = "{Origin of the X-ray disc-reflection steep radial emissivity}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1208.0360},
 primaryClass = "astro-ph.HE",
 keywords = {black hole physics, accretion, accretion disks, relativistic, processes, galaxies: nuclei},
     year = 2012,
    month = sep,
   volume = 545,
      eid = {A106},
    pages = {A106},
      doi = {10.1051/0004-6361/201219701},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...545A.106S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Thorne1975,
	author = {{Thorne}, K.~S. and {Price}, R.~H.},
	title = "{Cygnus X-1 - an interpretation of the spectrum and its variability}",
	journal = {\apjl},
	keywords = {Astronomical Models, Black Holes (Astronomy), Stellar Spectra, Variable Stars, X Ray Astronomy, X Ray Stars, Radiant Flux Density, Stellar Evolution, Stellar Rotation, X Ray Spectra},
	year = 1975,
	month = feb,
	volume = 195,
	pages = {L101-L105},
	doi = {10.1086/181720},
	adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...195L.101T},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Taylor2018a,
   author = {{Taylor}, C. and {Reynolds}, C.~S.},
    title = "{Exploring the Effects of Disk Thickness on the Black Hole Reflection Spectrum}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1712.05418},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, black hole physics, galaxies: active, galaxies: nuclei, galaxies: Seyfert, X-rays: galaxies},
     year = 2018,
    month = mar,
   volume = 855,
      eid = {120},
    pages = {120},
      doi = {10.3847/1538-4357/aaad63},
   adsurl = {http://adsabs.harvard.edu/abs/2018ApJ...855..120T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Taylor2018b,
   author = {{Taylor}, C. and {Reynolds}, C.~S.},
    title = "{X-Ray Reverberation from Black Hole Accretion Disks with Realistic Geometric Thickness}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1808.07877},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, black hole physics, galaxies: active, galaxies: nuclei, galaxies: Seyfert, X-rays: galaxies },
     year = 2018,
    month = dec,
   volume = 868,
      eid = {109},
    pages = {109},
      doi = {10.3847/1538-4357/aae9f2},
   adsurl = {http://adsabs.harvard.edu/abs/2018ApJ...868..109T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tomsick2014,
	author = {{Tomsick}, J.~A. and {Nowak}, M.~A. and {Parker}, M. and {Miller}, J.~M. and 
	{Fabian}, A.~C. and {Harrison}, F.~A. and {Bachetti}, M. and 
	{Barret}, D. and {Boggs}, S.~E. and {Christensen}, F.~E. and 
	{Craig}, W.~W. and {Forster}, K. and {F{\"u}rst}, F. and {Grefenstette}, B.~W. and 
	{Hailey}, C.~J. and {King}, A.~L. and {Madsen}, K.~K. and {Natalucci}, L. and 
	{Pottschmidt}, K. and {Ross}, R.~R. and {Stern}, D. and {Walton}, D.~J. and 
	{Wilms}, J. and {Zhang}, W.~W.},
	title = "{The Reflection Component from Cygnus X-1 in the Soft State Measured by NuSTAR and Suzaku}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1310.3830},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion disks, black hole physics, stars: individual: Cygnus X-1, X-rays: general, X-rays: stars },
	year = 2014,
	month = jan,
	volume = 780,
	eid = {78},
	pages = {78},
	doi = {10.1088/0004-637X/780/1/78},
	adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...780...78T},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tomsick2018,
   author = {{Tomsick}, J.~A. and {Parker}, M.~L. and {Garc{\'{\i}}a}, J.~A. and 
	{Yamaoka}, K. and {Barret}, D. and {Chiu}, J.-L. and {Clavel}, M. and 
	{Fabian}, A. and {F{\"u}rst}, F. and {Gandhi}, P. and {Grinberg}, V. and 
	{Miller}, J.~M. and {Pottschmidt}, K. and {Walton}, D.~J.},
    title = "{Alternative Explanations for Extreme Supersolar Iron Abundances Inferred from the Energy Spectrum of Cygnus X-1}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1801.07267},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, black hole physics, stars: individual: Cygnus X-1, X-rays: general, X-rays: stars},
     year = 2018,
    month = mar,
   volume = 855,
      eid = {3},
    pages = {3},
      doi = {10.3847/1538-4357/aaaab1},
   adsurl = {http://adsabs.harvard.edu/abs/2018ApJ...855....3T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Uttley2005,
	author = {{Uttley}, P. and {McHardy}, I.~M. and {Vaughan}, S.},
	title = "{Non-linear X-ray variability in X-ray binaries and active galaxies}",
	journal = {\mnras},
	eprint = {astro-ph/0502112},
	keywords = {methods: data analysis, methods: statistical, galaxies: active, X-rays: binaries, X-rays: galaxies, X-rays: individual: Cygnus X-1},
	year = 2005,
	month = may,
	volume = 359,
	pages = {345-362},
	doi = {10.1111/j.1365-2966.2005.08886.x},
	adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.359..345U},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Uttley2011,
	author = {{Uttley}, P. and {Wilkinson}, T. and {Cassatella}, P. and {Wilms}, J. and 
	{Pottschmidt}, K. and {Hanke}, M. and {B{\"o}ck}, M.},
	title = "{The causal connection between disc and power-law variability in hard state black hole X-ray binaries}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1104.0634},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual: GX 339-4},
	year = 2011,
	month = jun,
	volume = 414,
	pages = {L60-L64},
	doi = {10.1111/j.1745-3933.2011.01056.x},
	adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414L..60U},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Uttley2014,
	author = {{Uttley}, P. and {Cackett}, E.~M. and {Fabian}, A.~C. and {Kara}, E. and 
	{Wilkins}, D.~R.},
	title = "{X-ray reverberation around accreting black holes}",
	journal = {\aapr},
	archivePrefix = "arXiv",
	eprint = {1405.6575},
	primaryClass = "astro-ph.HE",
	keywords = {Accretion, accretion disks, Black hole physics, Galaxies: active, Galaxies: Seyfert, X-rays: binaries},
	year = 2014,
	month = aug,
	volume = 22,
	eid = {72},
	pages = {72},
	doi = {10.1007/s00159-014-0072-0},
	adsurl = {http://adsabs.harvard.edu/abs/2014A%26ARv..22...72U},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vaughan1997,
	author = {{Vaughan}, B.~A. and {Nowak}, M.~A.},
	title = "{X-Ray Variability Coherence: How to Compute It, What It Means, and How It Constrains Models of GX 339-4 and Cygnus X-1}",
	journal = {\apjl},
	eprint = {astro-ph/9610257},
	keywords = {BLACK HOLE PHYSICS, METHODS: STATISTICAL, X-RAYS: STARS, Black Hole Physics, Methods: Statistical, X-Rays: Stars},
	year = 1997,
	month = jan,
	volume = 474,
	pages = {L43-L46},
	doi = {10.1086/310430},
	adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...474L..43V},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Veledina2018,
   author = {{Veledina}, A.},
    title = "{Interplay of spectral components in timing properties of accreting compact objects}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1809.06053},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, X-rays: binaries},
     year = 2018,
    month = dec,
   volume = 481,
    pages = {4236-4249},
      doi = {10.1093/mnras/sty2556},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.481.4236V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jiang2019,
   author = {{Jiang}, J. and {Fabian}, A.~C. and {Wang}, J. and {Walton}, D.~J. and 
	{Garc{\'{\i}}a}, J.~A. and {Parker}, M.~L. and {Steiner}, J.~F. and 
	{Tomsick}, J.~A.},
    title = "{High-density reflection spectroscopy: I. A case study of GX 339-4}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1901.01739},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual (GX 339-4)},
     year = 2019,
    month = apr,
   volume = 484,
    pages = {1972-1982},
      doi = {10.1093/mnras/stz095},
   adsurl = {http://adsabs.harvard.edu/abs/2019MNRAS.484.1972J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Walton2013,
   author = {{Walton}, D.~J. and {Zoghbi}, A. and {Cackett}, E.~M. and {Uttley}, P. and 
	{Harrison}, F.~A. and {Fabian}, A.~C. and {Kara}, E. and {Miller}, J.~M. and 
	{Reis}, R.~C. and {Reynolds}, C.~S.},
    title = "{Hard X-Ray Lags in Active Galactic Nuclei: Testing the Distant Reverberation Hypothesis with NGC 6814}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1310.0822},
 primaryClass = "astro-ph.HE",
 keywords = {black hole physics, galaxies: active, X-rays: individual: NGC 6814},
     year = 2013,
    month = nov,
   volume = 777,
      eid = {L23},
    pages = {L23},
      doi = {10.1088/2041-8205/777/2/L23},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...777L..23W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Walton2016,
   author = {{Walton}, D.~J. and {Tomsick}, J.~A. and {Madsen}, K.~K. and 
	{Grinberg}, V. and {Barret}, D. and {Boggs}, S.~E. and {Christensen}, F.~E. and 
	{Clavel}, M. and {Craig}, W.~W. and {Fabian}, A.~C. and {Fuerst}, F. and 
	{Hailey}, C.~J. and {Harrison}, F.~A. and {Miller}, J.~M. and 
	{Parker}, M.~L. and {Rahoui}, F. and {Stern}, D. and {Tao}, L. and 
	{Wilms}, J. and {Zhang}, W.},
    title = "{The Soft State of Cygnus X-1 Observed with NuSTAR: A Variable Corona and a Stable Inner Disk}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1605.03966},
 primaryClass = "astro-ph.HE",
 keywords = {black hole physics, X-rays: binaries, X-rays: individual: Cygnus X-1},
     year = 2016,
    month = jul,
   volume = 826,
      eid = {87},
    pages = {87},
      doi = {10.3847/0004-637X/826/1/87},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...826...87W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilkins2013,
	author = {{Wilkins}, D.~R. and {Fabian}, A.~C.},
	title = "{The origin of the lag spectra observed in AGN: Reverberation and the propagation of X-ray source fluctuations}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1212.2213},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, black hole physics, galaxies: active, X-rays: galaxies},
	year = 2013,
	month = mar,
	volume = 430,
	pages = {247-258},
	doi = {10.1093/mnras/sts591},
	adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.430..247W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilkins2015,
       author = {{Wilkins}, D.~R. and {Gallo}, L.~C.},
        title = "{Driving extreme variability: the evolving corona and evidence for jet launching in Markarian 335}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, galaxies: active, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2015",
        month = "May",
       volume = {449},
       number = {1},
        pages = {129-146},
          doi = {10.1093/mnras/stv162},
archivePrefix = {arXiv},
       eprint = {1501.05302},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.449..129W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilkins2016,
	author = {{Wilkins}, D.~R. and {Cackett}, E.~M. and {Fabian}, A.~C. and 
	{Reynolds}, C.~S.},
	title = "{Towards modelling X-ray reverberation in AGN: piecing together the extended corona}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1602.00022},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, black hole physics, galaxies: active, X-rays: galaxies},
	year = 2016,
	month = may,
	volume = 458,
	pages = {200-225},
	doi = {10.1093/mnras/stw276},
	adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.458..200W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilkinson2009,
	author = {{Wilkinson}, T. and {Uttley}, P.},
	title = "{Accretion disc variability in the hard state of black hole X-ray binaries}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {0905.0587},
	primaryClass = "astro-ph.HE",
	keywords = {black hole physics , methods: statistical , X-rays: binaries},
	year = 2009,
	month = aug,
	volume = 397,
	pages = {666-676},
	doi = {10.1111/j.1365-2966.2009.15008.x},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.397..666W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilms2000,
	author = {{Wilms}, J. and {Allen}, A. and {McCray}, R.},
	title = "{On the Absorption of X-Rays in the Interstellar Medium}",
	journal = {\apj},
	eprint = {astro-ph/0008425},
	keywords = {Atomic Data, ISM: Dust, Extinction, ISM: Abundances, X-Rays: ISM},
	year = 2000,
	month = oct,
	volume = 542,
	pages = {914-924},
	doi = {10.1086/317016},
	adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...542..914W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilms2006,
	author = {{Wilms}, J. and {Nowak}, M.~A. and {Pottschmidt}, K. and {Pooley}, G.~G. and 
	{Fritz}, S.},
	title = "{Long term variability of Cygnus X-1. IV. Spectral evolution 1999-2004}",
	journal = {\aap},
	eprint = {astro-ph/0510193},
	keywords = {stars: individual: Cyg X-1, stars: binaries: close, X-rays: binaries, black hole physics},
	year = 2006,
	month = feb,
	volume = 447,
	pages = {245-261},
	doi = {10.1051/0004-6361:20053938},
	adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...447..245W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zdziarski1996,
   author = {{Zdziarski}, A.~A. and {Johnson}, W.~N. and {Magdziarz}, P.},
    title = "{Broad-band {$\gamma$}-ray and X-ray spectra of NGC 4151 and their implications for physical processes and geometry.}",
  journal = {\mnras},
   eprint = {astro-ph/9607015},
 keywords = {galaxies: individual: NGC4151 -- galaxies: Seyfert -- gamma-rays: observations -- gamma-rays: theory X-rays: galaxies, Seyfert Galaxies: X-Ray Spectra, Seyfert Galaxies: Gamma-Ray Spectra, Seyfert Galaxies: Radiation Mechanisms},
     year = 1996,
    month = nov,
   volume = 283,
    pages = {193-206},
      doi = {10.1093/mnras/283.1.193},
   adsurl = {http://adsabs.harvard.edu/abs/1996MNRAS.283..193Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zdziarski2003,
	author = {{Zdziarski}, A.~A. and {Lubi{\'n}ski}, P. and {Gilfanov}, M. and 
	{Revnivtsev}, M.},
	title = "{Correlations between X-ray and radio spectral properties of accreting black holes}",
	journal = {\mnras},
	eprint = {astro-ph/0209363},
	keywords = {accretion, accretion discs, radiation mechanisms: thermal, binaries: general, galaxies: Seyfert, X-rays: galaxies, X-rays: stars},
	year = 2003,
	month = jun,
	volume = 342,
	pages = {355-372},
	doi = {10.1046/j.1365-8711.2003.06556.x},
	adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.342..355Z},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zycky1999,
   author = {{{\.Z}ycki}, P.~T. and {Done}, C. and {Smith}, D.~A.},
    title = "{The 1989 May outburst of the soft X-ray transient GS 2023+338 (V404 Cyg)}",
  journal = {\mnras},
   eprint = {astro-ph/9904304},
     year = 1999,
    month = nov,
   volume = 309,
    pages = {561-575},
      doi = {10.1046/j.1365-8711.1999.02885.x},
   adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.309..561Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zoghbi2010,
       author = {{Zoghbi}, A. and {Fabian}, A.~C. and {Uttley}, P. and {Miniutti}, G. and
         {Gallo}, L.~C. and {Reynolds}, C.~S. and {Miller}, J.~M. and
         {Ponti}, G.},
        title = "{Broad iron L line and X-ray reverberation in 1H0707-495}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: individual: 1H0707-495, galaxies: nuclei, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = feb,
       volume = {401},
       number = {4},
        pages = {2419-2432},
          doi = {10.1111/j.1365-2966.2009.15816.x},
archivePrefix = {arXiv},
       eprint = {0910.0367},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.401.2419Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zoghbi2011,
	author = {{Zoghbi}, A. and {Uttley}, P. and {Fabian}, A.~C.},
	title = "{Understanding reverberation lags in 1H0707-495}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1010.3744},
	primaryClass = "astro-ph.HE",
	keywords = {galaxies: active, galaxies: individual: 1H0707-495, galaxies: nuclei, X-rays: galaxies},
	year = 2011,
	month = mar,
	volume = 412,
	pages = {59-64},
	doi = {10.1111/j.1365-2966.2010.17883.x},
	adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.412...59Z},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zoghbi2012,
   author = {{Zoghbi}, A. and {Fabian}, A.~C. and {Reynolds}, C.~S. and {Cackett}, E.~M.},
    title = "{Relativistic iron K X-ray reverberation in NGC 4151}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1112.1717},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, X-rays: galaxies},
     year = 2012,
    month = may,
   volume = 422,
    pages = {129-134},
      doi = {10.1111/j.1365-2966.2012.20587.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422..129Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zoghbi2014,
       author = {{Zoghbi}, A. and {Cackett}, E.~M. and {Reynolds}, C. and {Kara}, E. and
         {Harrison}, F.~A. and {Fabian}, A.~C. and {Lohfink}, A. and {Matt}, G. and
         {Balokovic}, M. and {Boggs}, S.~E. and {Christensen}, F.~E. and
         {Craig}, W. and {Hailey}, C.~J. and {Stern}, D. and {Zhang}, W.~W.},
        title = "{Observations of MCG-5-23-16 with Suzaku, XMM-Newton and NuSTAR: Disk Tomography and Compton Hump Reverberation}",
      journal = {\apj},
     keywords = {galaxies: active, X-rays: galaxies, X-rays: individual: MCG-5-23-16, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = jul,
       volume = {789},
       number = {1},
          eid = {56},
        pages = {56},
          doi = {10.1088/0004-637X/789/1/56},
archivePrefix = {arXiv},
       eprint = {1405.3674},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...789...56Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zoghbi2020,
       author = {{Zoghbi}, Abderahmen and {Kalli}, Sihem and {Miller}, Jon M. and
         {Mizumoto}, Misaki},
        title = "{Testing the Lamp-post and Wind Reverberation Models with XMM-Newton Observations of NGC 5506}",
      journal = {\apj},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = apr,
       volume = {893},
       number = {2},
          eid = {97},
        pages = {97},
          doi = {10.3847/1538-4357/ab7dc8},
archivePrefix = {arXiv},
       eprint = {2003.04322},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...893...97Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





